Deeply Inelastic Scattering Revisited

Due to its conceptual simplicity, Deeply Inelastic Scattering (DIS) often serves as a textbook example for Quantum Chromo Dynamics (QCD) and partonic structure of nucleons. However, it is this supposed simplicity, which makes DIS an ideal case for discussing many additional effects and corrections. In these lectures we discuss DIS within the domain of perturbative QCD covering a range of topics ranging from mathematical problems to kinematical corrections, and to practical challenges when attempting to interpret experimental measurements. Although here we focus on the exemplary case of DIS, the discussed topcis are relevant to a larger class of processes. We also give an overview of existing and future DIS measurements, and discuss their implementation into modern extractions of parton distribution functions (PDFs) which quantify the partonic structure of nucleons. The discussed features are all implemented in the open source code Yadism, which has been used for PDF extractions from a wide range of the available world data on fully inclusive DIS.

==> preamble.tex <==
\usepackage{xspace}
%
%
\usepackage{subcaption}
%
\usepackage{bbm}
\usepackage{verbatim}
\usepackage{amssymb}

%
%
\usepackage[english]{babel}
\selectlanguage{english}

%
\RequirePackage{cite}
%
%

%
%
\RequirePackage[colorlinks=true,bookmarks=true,plainpages=false
%
%
%
%
%
%
%
%
%
]{hyperref}
\RequirePackage[capitalise]{cleveref}


\RequirePackage[status=draft,inline,nomargin,marginclue]{fixme}
%
\fxusetheme{color}
%
\FXRegisterAuthor{fh}{afh}{FH}
\RequirePackage{tcolorbox}
\newtcolorbox[auto counter,number within=chapter,crefname={conclusion}{conclusions}]{conclusionbox}[2][]{%
%
title=Conclusion~\thetcbcounter: #2,#1}
\newtcolorbox[auto counter,number within=section,crefname={exercise}{exercises}]{exercisebox}[2][]{%
colback=white,%
title=Exercise~\thetcbcounter: #2,#1}

%

%
\RequirePackage{hepnames}
\RequirePackage{hepunits}
\usepackage{slashed}

\RequirePackage{siunitx}
\RequirePackage{physics}
\sisetup{
    retain-unity-mantissa = false
}
%

\DeclareRobustCommand{\LQCD}[0]{\Lambda_\text{QCD}}
\DeclareRobustCommand{\aem}[0]{\alpha_\text{em}}
\DeclareRobustCommand{\msbar}[0]{\overline{\mathrm{MS}}}

